Semantic-Aware Task Clustering for Constructive and Cooperative Multi-Tasking

Cooperative multi-task semantic communication (CMT-SemCom) improves task execution performance by leveraging shared representations. However, as we demonstrated in [1], cooperative multi-tasking can be either constructive or destructive, depending on the semantic relationships among tasks. To ensure constructive cooperation, we propose a semantic-aware task clustering method for CMT-SemCom. We have formulated a sequential multi-stage optimization problem in which semantically aligned tasks are clustered once after a short initial training phase, and then end-to-end (E2E) joint training is conducted exclusively within the discovered groups. Specifically, the problem decomposes into two stages: (i) a semantic clustering problem leveraging hierarchical density-based spatial clustering, and (ii) an intra-cluster E2E CMT-SemCom learning problem. Simulation results demonstrate that the proposed framework effectively mitigates destructive cooperation and negative transfer, yielding accuracy gains compared to unclustered multi-tasking and individual training baselines.

==> math_macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro definitions for mathematical symbols and functions                    %
%                                                                             %
% Author: C. Bockelmann (updated: 18.02.2011)                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathe.tex - Mathematische (Mengen)Zeichen, Symbole und Funktionen
%             fuer LaTeX 2.09 und LaTeX 2e
%
%             Original von Dieter Boss, 08/94
%             Letzte Aenderung: H.Schmidt, 26-April-2000 (NDFT ... NIFFT)
%
%	     bearbeitet von Henning Paul 11/07 und abgelegt als mymathe.tex
%
%	     zurechtgestutzt von Henning Paul 12/09, 01/12
%
% 		 bearbeitet von Ban-Sok Shin 03/22

% #####  Haeufig benoetigte Funktionen  #####
% \newacro{ATC-FWI}[ATC-FWI]{Adapt-Then-Combine Full Waveform Inversion}
% \newacro{FWI}[FWI]{Full Waveform Inversion}
% \newacro{NN}[NN]{Neural Network}
% \newacro{ML}[ML]{Machine Learning}
% \newacro{JSCC}[JSCC]{Joint Source and Channel Coding}
% \newacro{FL}[FL]{Federated Learning}
% \newacro{OAC}[AirComp]{Over-the-Air Computation}
% \newacro{ELBO}[ELBO]{Evidence Lower BOund}
% \newacro{MILBO}[MILBO]{Mutual Information Lower BOund}
% \newacro{dELBO}[dELBO]{Distributed Evidence Lower BOund}
% \newacro{dMILBO}[dMILBO]{Distributed Mutual Information Lower BOund}
% \newacro{AWGN}[AWGN]{Additive White Gaussian Noise}
% \newacro{DNN}[DNN]{Deep Neural Network}
% \newacro{SGD}[SGD]{Stochastic Gradient Descent}
% \newacro{MSE}[MSE]{Mean Square Error}
% \newacro{MAS}[MAS]{multi-agent system}  %{Multi Agent System}
% \newacro{CNN}[CNN]{Convolutional Neural Network}
% \newacro{NMSE}[NMSE]{Normalized Mean Square Error}
% \newacro{SSIM}[SSIM]{Structural Similarity Index Measure}
% \newacro{ViT}[ViT]{Vision Transformer}
% \newacro{ResNet}[ResNet]{Residual Network}
% \newacro{PReLU}[PReLU]{Parametric Rectified Linear Unit}
% \newacro{MSE}[MSE]{Mean Square Error}
% \newacro{NN}[NN]{Neural Network}
% \newacro{PSNR}[PSNR]{Peak Signal to Noise Ratio}
% \newacro{SNR}[SNR]{Signal to Noise Ratio}
% \newcommand{\s}{s}
% \newacro{pdf}[PDF]{Probability Density Function}
% \newacro{UMAP}[UMAP]{Uniform Manifold Approximation and Projection}
% \newacro{t-SNE}[t-SNE]{t-distributed Stochastic Neighbor Embedding} 




% Acronmy clickable setup
% \usepackage{ifthen}

% \acsetup{
%     first-style = long-short
% }

% \let\oldac\ac
% \let\oldacs\acs
% \let\oldacf\acf

% \makeatletter
% \RenewDocumentCommand{\ac}{m}{%
%   \@ifundefined{myac@#1@seen}{%
%     % First occurrence
%     \global\@namedef{myac@#1@seen}{}%
%     \leavevmode
%     \raisebox{1em}{\hypertarget{#1-first}{}}%
%     \oldacf{#1}%
%   }{%
%     % Later occurrences
%     \hyperlink{#1-first}{\oldacs{#1}}%
%   }%
% }
% \makeatother





% ----- Acronym definitions -----
\DeclareAcronym{ATC-FWI}{
    short = ATC-FWI,
    long  = Adapt-Then-Combine Full Waveform Inversion
}
\DeclareAcronym{FWI}{
    short = FWI,
    long  = Full Waveform Inversion
}
\DeclareAcronym{NN}{
    short = NN,
    long  = Neural Network
}
\DeclareAcronym{ML}{
    short = ML,
    long  = Machine Learning
}
\DeclareAcronym{JSCC}{
    short = JSCC,
    long  = Joint Source and Channel Coding
}
\DeclareAcronym{FL}{
    short = FL,
    long  = Federated Learning
}
\DeclareAcronym{OAC}{
    short = AirComp,
    long  = Over-the-Air Computation
}
\DeclareAcronym{ELBO}{
    short = ELBO,
    long  = Evidence Lower BOund
}
\DeclareAcronym{MILBO}{
    short = MILBO,
    long  = Mutual Information Lower BOund
}
\DeclareAcronym{dELBO}{
    short = dELBO,
    long  = Distributed Evidence Lower BOund
}
\DeclareAcronym{dMILBO}{
    short = dMILBO,
    long  = Distributed Mutual Information Lower BOund
}
\DeclareAcronym{AWGN}{
    short = AWGN,
    long  = Additive White Gaussian Noise
}
\DeclareAcronym{DNN}{
    short = DNN,
    long  = Deep Neural Network
}
\DeclareAcronym{SGD}{
    short = SGD,
    long  = Stochastic Gradient Descent
}
\DeclareAcronym{MSE}{
    short = MSE,
    long  = Mean Square Error
}
\DeclareAcronym{MAS}{
    short = MAS,
    long  = multi-agent system
}
\DeclareAcronym{CNN}{
    short = CNN,
    long  = Convolutional Neural Network
}
\DeclareAcronym{NMSE}{
    short = NMSE,
    long  = Normalized Mean Square Error
}
\DeclareAcronym{SSIM}{
    short = SSIM,
    long  = Structural Similarity Index Measure
}
\DeclareAcronym{ViT}{
    short = ViT,
    long  = Vision Transformer
}
\DeclareAcronym{ResNet}{
    short = ResNet,
    long  = Residual Network
}
\DeclareAcronym{PReLU}{
    short = PReLU,
    long  = Parametric Rectified Linear Unit
}
\DeclareAcronym{PSNR}{
    short = PSNR,
    long  = Peak Signal to Noise Ratio
}
\DeclareAcronym{SNR}{
    short = SNR,
    long  = Signal to Noise Ratio
}
\DeclareAcronym{pdf}{
    short = PDF,
    long  = Probability Density Function
}
\DeclareAcronym{UMAP}{
    short = UMAP,
    long  = Uniform Manifold Approximation and Projection
}
\DeclareAcronym{t-SNE}{
    short = t-SNE,
    long  = t-distributed Stochastic Neighbor Embedding
}
\DeclareAcronym{HDBSCAN}{
    short = HDBSCAN,
    long  = Hierarchical Density-Based Spatial Clustering of Applications with Noise
}



\newcommand{\weightSSIM}{\ensuremath{w_{i_n}}}  
\newcommand{\expct}{\ensuremath{\mathrm{E}}}
\newcommand{\entropy}{\ensuremath{\mathrm{H}}}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ld}{\ensuremath{\mathrm{ld}}}  
\newcommand{\erf}{\ensuremath{\mathrm{erf}}}
\newcommand{\erfc}{\ensuremath{\mathrm{erfc}}}
\newcommand{\ex}[1]{\ensuremath{\mathrm{e}^{#1}}}
\newcommand{\expc}[1]{\ensuremath{\mathrm{E}\left\{#1\right\}}}
\newcommand{\exj}[1]{\ensuremath{\mathrm{e}^{\mathrm{j}#1}}}
\newcommand{\exmj}[1]{\ensuremath{\mathrm{e}^{-\mathrm{j}#1}}}
\newcommand{\ejO}{\ex{\mathrm{j}\Omega}}
\newcommand{\jomega}{\ensuremath{\mathrm{j}\omega}}
\newcommand{\jnull}{\ensuremath{\mathrm{j}0}}

\newcommand{\herm}{\ensuremath{\mathrm{H}}}
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}}
\newcommand{\sgn}{\ensuremath{\mathrm{sgn}}}

\newcommand{\Matlab}{{\sc Matlab}}


% #####  Mengenzeichen  #####
\newcommand{\R}{\mathbb{R}} 
\newcommand{\C}{\mathbb{C}} 
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

%% #####  Worte, die haeufig in Gleichungen gebraucht werden  #####
%\newcommand{\Mit}{\quad\mathrm{mit}\;\,}          % kleingeschrieben existiert \mit schon!
%\newcommand{\und}{\quad\mathrm{und}\;\,}
%\newcommand{\da}{\quad\mathrm{da}\;\,}
%\newcommand{\fuer}{\quad\mathrm{f"ur}\;\,}
%\newcommand{\wobei}{\quad\mathrm{wobei}\;\,}
%\newcommand{\mindex}[1]{\mbox{\scriptsize \sl #1}}

% #####  Fettschrift fuer Vektoren  #####
\newcommand{\V}[1]{\ensuremath{\mathbf{#1}}}    % (fette) Vektoren oder Matrizen (mit Buchstabe als Argument)
\newcommand{\vek}[1]{\ensuremath{\mathbf{#1}}}    % (fette) Vektoren oder Matrizen (mit Buchstabe als Argument)
\newcommand{\vsym}[1]{\ensuremath{\boldsymbol{#1}}}    % (fette) Vektoren oder Matrizen (mit Symbol als Argument)
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}    % (fette) Vektoren oder Matrizen (mit Buchstabe als Argument)
\newcommand{\bs}[1]{\mbox{\boldmath$#1$}}         % (fette) schraege Vektoren oder Matrizen

% ######################################

\DeclareMathAlphabet\mathboldsf{OT1}{cmss}{bx}{n} 
\newcommand{\veks}[1]{\ensuremath{\mathboldsf{#1}}}

\renewcommand {\Re}[1]{{\mathrm{Re}\left\{#1\right\}}} % Realteil
\renewcommand {\Im}[1]{{\mathrm{Im}\left\{#1\right\}}} % Imaginaerteil

% Abbreviations in math formulas
\newcommand{\FWI}{\mathrm{FWI}}  % full waveform inversion
\newcommand{\TT}{\mathrm{TT}} % traveltime tomography

\newcommand{\re}{\mathrm{Re}} % Realteil
\newcommand{\im}{\mathrm{Im}} % Imaginaerteil

\newcommand{\Ra}[1]{{\mathrm{Ra}\left\{#1\right\}}} 
\newcommand{\Ia}[1]{{\mathrm{Ia}\left\{#1\right\}}}
\newcommand{\diag}[1]{{\mathrm{diag}(#1)}}
\newcommand{\xpt}[1]{\mathrm{E}\left\{#1\right\}}
\newcommand{\xptH}[1]{\mathrm{E}_\veks{H}\left\{#1\right\}}
\newcommand{\trace}[1]{\mathrm{tr}\left\{#1\right\}}
\newcommand{\vnorm}[1]{\left\|#1\right\|}
\newcommand{\h}{\mathsf{H}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\inv}[1]{#1^{-1}} % inverse of anything
\newcommand{\spalw}[1]{\mathrm{vec}\left\{#1\right\}}
\newcommand{\rank}[1]{\mathrm{rank}\left\{#1\right\}}

\newcommand{\centmin}{\operatornamewithlimits{min}}
\newcommand{\centmax}{\operatornamewithlimits{max}}

% Klammern
\newcommand{\rund}[1]{\left(#1\right)}
\newcommand{\eckig}[1]{\left[#1\right]}
\newcommand{\curly}[1]{\left\{#1\right\}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

% Einheiten
\newcommand{\ms}{\milli\second}
\newcommand{\mm}{\milli\meter}
\newcommand{\cm}{\centi\meter}
\newcommand{\km}{\kilo\meter}
\newcommand{\hz}{\hertz}
\newcommand{\mhz}{\mega\hertz}
\newcommand{\ghz}{\giga\hertz}
\newcommand{\db}{\deci\bel}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

% \newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}

% text
\newcommand{\obs}{\ensuremath{\mathrm{obs}}}
\newcommand{\syn}{\ensuremath{\mathrm{syn}}}
\newcommand{\iter}{\ensuremath{k}}
\newcommand{\itn}{\ensuremath{{[\iter]}}}
\newcommand{\itup}{\ensuremath{{[\iter+1]}}}
\newcommand{\ADMM}{\mathrm{ADMM}}
\newcommand{\TOMO}{\mathrm{TOMO}}

% operators
\newcommand{\inprod}[1]{\left\langle#1\right\rangle}
\newcommand{\ndegree}{\delta}
\newcommand{\ndegreeNode}{\ndegree_{\idxNode}}
%\newcommand{\argmin}{\text{argmin}}
\newcommand{\grad}{\nabla}
\newcommand{\drm}{\mathrm{d}}

% dimensions
\newcommand{\Nx}{{\ensuremath{N_{\mathrm{x}}}}}
\newcommand{\Ny}{{\ensuremath{N_{\mathrm{y}}}}}
\newcommand{\Nz}{{\ensuremath{N_{\mathrm{z}}}}}

% constants
\newcommand{\noGen}{M}
\newcommand{\noRec}{{\ensuremath{N_{\mathrm{R}}}}}
\newcommand{\noSrc}{{\ensuremath{N_{\mathrm{S}}}}}
\newcommand{\noTime}{{\ensuremath{N_{\mathrm{T}}}}}

% indices
\newcommand{\idxRec}{r}
\newcommand{\idxSrc}{s}
\newcommand{\idxGen}{m}
\newcommand{\idxIter}{k}
\newcommand{\idxNode}{j}
\newcommand{\idxNeigh}{\ell}
\newcommand{\idxNodeNeigh}{{\idxRec\idxNeigh}}
\newcommand{\idxNeighNode}{{\idxNeigh\idxRec}}

% functions

% sets
\newcommand{\setNeighAug}{\mathcal{N}'}
\newcommand{\setNeigh}{\mathcal{N}}
\newcommand{\setNeighNode}{\mathcal{N}_{\idxRec}}
\newcommand{\setNodes}{\mathcal{J}}
\newcommand{\setRecs}{\mathcal{R}}
\newcommand{\setEdges}{\mathcal{E}}
\newcommand{\setGraph}{\mathcal{G}}

% Functions
\newcommand{\lcost}{\ensuremath{\mathcal{J}}}
\newcommand{\cost}{\ensuremath{\mathcal{L}}}
\newcommand{\kernel}{\ensuremath{\kappa}}
\newcommand{\wavefield}{\ensuremath{u}}
\newcommand{\slowness}{\ensuremath{m}}
\newcommand{\source}{\ensuremath{f}}

\newcommand{\stepSize}{\ensuremath{\alpha}}
\newcommand{\stepAdmm}{\ensuremath{\varepsilon}}
\newcommand{\stdev}{\ensuremath{\sigma}}
\newcommand{\variance}{\stdev^2}
% input/output data, variables
\newcommand{\eigenVal}{\lambda}

\newcommand{\freqRad}{\omega}
\newcommand{\freqF}{f}
\newcommand{\model}{\ensuremath{m}}
\newcommand{\scaTravTime}{\ensuremath{T}}
\newcommand{\scaTravTimeRes}{\rho}
\newcommand{\scaWeight}{w}
\newcommand{\scaData}{d}
\newcommand{\scaOutputTime}{\scaOutput_\idxIter}
\newcommand{\scaOutputNode}{\scaOutput_{\idxNode}}
\newcommand{\scaOutputNodeTime}{\scaOutput_{\idxNode,\idxIter}}
\newcommand{\scaOutputNeigh}{\scaOutput_{\idxNeigh}}
\newcommand{\scaOutputNeighTime}{\scaOutput_{\idxNeigh,\idxIter}}
\newcommand{\scaOutputEst}{\hat{\scaOutput}}
\newcommand{\scaInput}{x}
\newcommand{\scaReflect}{h}
\newcommand{\scaNoise}{n}
\newcommand{\scaNoiseNode}{\scaNoise_{\idxNode}}
\newcommand{\scaNoiseNodeTime}{\scaNoise_{\idxNode,\idxIter}}
\newcommand{\scaWavelet}{w}
\newcommand{\scaError}{e}
\newcommand{\scaErrorTime}{\scaError_\idxIter}
%\newcommand{\scaErrorRKHS}{\varepsilon}
\newcommand{\scaCross}{r}
\newcommand{\scaEdge}{v}
\newcommand{\scaCoeff}{b}
\newcommand{\eigVal}{\lambda}

\newcommand{\adjoint}{\ensuremath{\uplambda}}

% variances
\newcommand{\noiseVar}{\variance_{\scaNoise}} % noise variance

\newcommand{\vecc}[1]{\vsym{#1}}
\newcommand{\vecWavefield}{\ensuremath{\vecc{\wavefield}}}
\newcommand{\vecSlowness}{\ensuremath{\vecc{\slowness}}}
\newcommand{\vecSource}{\ensuremath{\vecc{\source}}}

\newcommand{\vecTravTime}{\ensuremath{\vsym{\scaTravTime}}}
\newcommand{\vecTravTimeRes}{\vecc{\scaTravTimeRes}}
\newcommand{\vecModelGrad}{\vecc{\model}_\Delta}
\newcommand{\vecModel}{\ensuremath{\vsym{\model}}}
\newcommand{\vecCoord}{\ensuremath{\vsym{x}}}
\newcommand{\vecAdjoint}{\ensuremath{\vsym{\adjoint}}}
\newcommand{\vecWeight}{\ensuremath{\vsym{\scaWeight}}}
\newcommand{\vecWeightOpt}{\ensuremath{\vsym{\scaWeight}^\star}}

\newcommand{\vecData}{\vecc{\scaData}}
\newcommand{\vecOutputNode}{\vecOutput_{\idxNode}}
\newcommand{\vecOutputNeigh}{\vecOutput_{\idxNeigh}}
\newcommand{\vecOutputNodeTime}{\vecOutput_{\idxNode,\idxIter}}
\newcommand{\vecOutputNeighTime}{\vecOutput_{\idxNeigh,\idxIter}}
\newcommand{\vecOutputEst}{\vsym{\scaOutputEst}}
\newcommand{\vecInput}{\vsym{\scaInput}}
\newcommand{\vecInputNode}{\vecInput_{\idxNode}}
\newcommand{\vecInputTime}{\vecInput_{\idxIter}}
\newcommand{\vecWavelet}{\vsym{\scaWavelet}}
\newcommand{\vecReflect}{\vsym{\scaReflect}}
\newcommand{\vecNoise}{\vsym{\scaNoise}}

\newcommand{\vecCross}{\vecc{\scaCross}}
\newcommand{\vecCrossEst}{\hat{\vecc{\scaCross}}}
\newcommand{\vecOnes}{\vecc{1}}

\newcommand{\matForward}{\mathbf{A}}
\newcommand{\matEye}{\vsym{I}}
\newcommand{\matGram}{\vsym{G}}
\newcommand{\matReflect}{\vsym{H}}
\newcommand{\matConsensus}{\vsym{P}}
\newcommand{\matConsensusMod}{\widehat{\matConsensus}}
\newcommand{\matEdge}{\vecc{V}}

% parameters
\newcommand{\parCoh}{\delta_{\text{coh}}}
\newcommand{\parDis}{\delta_{\text{dis}}}
\newcommand{\parErr}{\delta_{\text{err}}}
\newcommand{\parSlab}{\varepsilon}
%\newcommand{\parSlab}{{\delta_{\text{slab}}}}
\newcommand{\parReg}{\epsilon}
\newcommand{\parRegNlms}{\parReg_{\mathrm{NLMS}}}
\newcommand{\parRegKnlms}{\parReg_{\mathrm{KNLMS}}}
\newcommand{\parRegMknlms}{\parReg_{\mathrm{MKNLMS}}}
\newcommand{\parRegHyp}{\parReg_{\mathrm{HYP}}}
\newcommand{\parRegChyp}{\parReg_{\mathrm{CHYP}}}


% hyperplanes, hyperslabs
\newcommand{\hslab}{\mathcal{S}}
\newcommand{\hslabNode}{\hslab_{\idxNode}}
\newcommand{\hslabNodeTime}{\hslab_{\idxNode,\idxIter}}
\newcommand{\hplane}{H}
\newcommand{\hplaneNode}{\hplane_{\idxNode}}
\newcommand{\hplaneNodeTime}{\hplane_{\idxNode,\idxIter}}

% DiCE
\newcommand{\scaLagrange}{u}
\newcommand{\scaAuxvar}{z}
\newcommand{\scaAuxvarNode}{\scaAuxvar_{\idxNode}}
\newcommand{\scaAuxvarNeigh}{\scaAuxvar_{\idxNeigh}}

\newcommand{\vecLagrange}{\vecc{\scaLagrange}}
\newcommand{\vecAuxvar}{\vecc{\scaAuxvar}}
\newcommand{\vecAuxvarNode}{\vecAuxvar_{\idxNode}}
\newcommand{\vecAuxvarNodeTime}{\vecAuxvar_{\idxNode,\idxIter}}
\newcommand{\vecAuxvarNeigh}{\vecAuxvar_{\idxNeigh}}
\newcommand{\vecAuxvarNeighTime}{\vecAuxvar_{\idxNeigh,\idxIter}}

% vector spaces
\newcommand{\spaceRKHS}{\mathcal{H}}
\newcommand{\spaceDict}{\mathcal{M}}
\newcommand{\spaceDictProd}{\spaceDict^{\times}}
\newcommand{\spaceDictSum}{\spaceDict^+}
\newcommand{\spaceFeature}{\mathcal{F}}
\newcommand{\spaceInput}{\mathcal{X}}
\newcommand{\spaceOutput}{\mathbb{R}}
\newcommand{\spaceSum}{\spaceRKHS^+}
\newcommand{\spaceProd}{\spaceRKHS^\times}
\newcommand{\spaceConsensus}{\mathcal{C}}
\newcommand{\spaceHilbert}{\mathbb{H}}





\newcommand{\legendfontsize}{\normalsize}
\newcommand{\ltickfontsize}{\tiny} % normalsize
\newcommand*{\labelaxisfontsize}{\small}


\newcommand{\markrepeat}{1}
\newcommand{\xminimum}{0}
\newcommand{\xmaximum}{0.7}
\newcommand{\yminimum}{-20}
\newcommand*{\ymaximum}{0}

\newcommand*{\nth}[2]{
    \foreach \xindx [count=\kcount from 0] in #1 {
        \ifnum\kcount=#2
            \xindx
        \fi
    }
}

\newcommand{\xlabel}{time$[dBdB]$}
\newcommand{\ylabel}{system mismatch $[dBdB]$}

\newboolean{xtickAutomatic}
\setboolean{xtickAutomatic}{true}
\newcommand{\xticklabelList}{0, 0.1, 0.3, 0.5}
\newboolean{ytickAutomatic}
\setboolean{ytickAutomatic}{true}
\newcommand{\yticklabelList}{0, 0.1, 0.3, 0.5}

\newboolean{xMinAutomatic}
\setboolean{xMinAutomatic}{true}
\newboolean{xMaxAutomatic}
\setboolean{xMaxAutomatic}{true}

\newboolean{yMinAutomatic}
\setboolean{yMinAutomatic}{true}
\newboolean{yMaxAutomatic}
\setboolean{yMaxAutomatic}{true}

\newboolean{LegendAutomatic}
\setboolean{LegendAutomatic}{true}

\newcommand{\legendnumbercolums}{1}
\newcommand{\legendtranspose}{ }
\newcommand{\legendlabela}{1}
\newcommand{\legendlabelb}{2}
\newcommand{\legendlabelc}{3}
\newcommand{\legendlabeld}{4}
\newcommand{\legendlabele}{5}
\newcommand{\legendlabelf}{6}
\newcommand{\legendlabelg}{7}
\newcommand{\legendlabelh}{8}
\newcommand{\legendlabeli}{9} 
\newcommand{\legendlabelj}{10}
\newcommand{\legendlabelk}{11}
\newcommand{\legendlabell}{12}
\newcommand{\legendlabelm}{13}
\newcommand{\legendlabeln}{14}

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "../diss"
%%% End: 

